DExperts: Decoding-Time Controlled Text Generation with Experts and Anti-Experts

Despite recent advances in natural language generation, it remains challenging to control attributes of generated text. We propose DExperts: Decoding-time Experts, a decoding-time method for controlled text generation that combines a pretrained language model with "expert" LMs and/or "anti-expert" LMs in a product of experts. Intuitively, under the ensemble, tokens only get high probability if they are considered likely by the experts, and unlikely by the anti-experts. We apply DExperts to language detoxification and sentiment-controlled generation, where we outperform existing controllable generation methods on both automatic and human evaluations. Moreover, because DExperts operates only on the output of the pretrained LM, it is effective with (anti-)experts of smaller size, including when operating on GPT-3. Our work highlights the promise of tuning small LMs on text with (un)desirable attributes for efficient decoding-time steering.

==> sections/old.5.analysis.tex <==
\section{Analysis}\label{sec:analysis}
In this section, we show that our method allows precise control over the tradeoff between style control and language fluency (\S\ref{subsec:hyperparameter_tuning}), requires much less stylistic data than existing methods (\S\ref{subsec:dataset_size}), and is effective at steering away from different, fine-grained notions of toxicity (\S\ref{subsec:customization}).
\maarten{not sure i like this conclusion-y sentence here?}
Together, these findings suggest that our method is extremely adaptable. 
For example, when a LM is in deployment, users can optionally flag output as examples of content that they do not want to see, which can be used to customize an anti-expert LM for each user. 
In contrast to training a classifier or a conditional LM with contrasting control codes, this does not require users to flag \textit{all} such unwanted examples, nor to label both positive and negative examples. 

\subsection{Hyperparameter tuning}\label{subsec:hyperparameter_tuning}
In \textsc{\methodName}, the hyperparameter $\alpha$ controls the amount of control over the base LM.
Figure \ref{fig:toxicity_hyperparam} illustrates the relationship between output fluency and toxicity for different choices of $\alpha$.
In our experiments, we pick $\alpha=2.0$ because it corresponds to the point where the curve flattens, indicating that further cost in fluency does not return as great of a reduction in toxicity. 
The smoothness of the tradeoff between detoxification and fluency indicates that $\alpha$ is a knob that users can control depending on their own application. 
The plot between sentiment control and fluency looks very similar for sentiment control experiments, and is included in Appendix \S\ref{sec:additional_results}.

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.4]{figures/toxicity_v_perplexity.png}
    \caption{The relationship between output fluency and toxicity for different values of the hyperparameter $\alpha$, which controls the amount of steering in our method. Results are calculated on a subset of 1K nontoxic prompts.}
    \label{fig:toxicity_hyperparam}
\end{figure}

\begin{table}[h!]
    \centering
    \small
    \begin{tabular}{cccccc}
    \toprule
        \multicolumn{2}{c}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{4}{c}{\textbf{Average max toxicity}} \\
        && \begin{tabular}{@{}c@{}}Identity\\attack\end{tabular} & Insult & \begin{tabular}{@{}c@{}}Sexually\\explicit\end{tabular} & Threat \\\midrule
        \multicolumn{2}{c}{GPT-2} & 0.432 & 0.476 & 0.408 & 0.593 \\\midrule
        \multirow{4}{*}{\rotatebox[origin=c]{90}{\methodName}} & \begin{tabular}{@{}c@{}}Identity\\attack\end{tabular} & \textbf{0.245} & 0.310 & 0.322 & 0.452 \\
        & Insult & 0.266 & \textbf{0.288} & 0.330 & 0.435 \\
        & \begin{tabular}{@{}c@{}}Sexually\\explicit\end{tabular} & 0.296 & 0.316 & \textbf{0.230} & 0.477 \\
        & Threat & 0.281 & 0.323 & 0.325 & \textbf{0.370} \\
    \bottomrule
    \end{tabular}
    \caption{Results when the anti-expert LM for language avoidance is specialized on fine-grained categories of toxic language.}
    \label{tab:toxicity_customization}
\end{table}

\subsection{Finetuning dataset size}\label{subsec:dataset_size}
In practice, gathering large amounts of toxic data may be challenging, especially in applications where we would want to customize the anti-expert LM for users who have differing notions of harmful language. 
To explore the limited data setting, we investigate the relationship between the dataset size used to train the toxic LM and its effectiveness as an anti-expert.
\maarten{Need a little more high level motivation here, that gathering large amounts of toxic data might be harder and people may want to update the anti-expert when they see something bad, so want to explore more limited data settings.}
% We investigate the relationship between the dataset size used to train the toxic LM and its effectiveness as an anti-expert in the ensemble. 
We train several toxic models on differently-sized subsets of the toxic training data, and use different checkpoints of each model as the anti-expert in our ensemble. 
With our finetuning hyperparameters (given in \S\ref{subsec:training_hyperparameters}), each update step consists of training on one batch of 512 tokens. 
We choose three dataset sizes: 51.2K tokens, 256K tokens, and 512K tokens (all exactly), corresponding to $200$ batches, $500$ batches, and $1000$ batches, respectively. 
(Recall that our full toxic dataset has $\sim$ 10M tokens.) 
We train each model for $3000$ steps. 
The performance of each model, at every $100$ update steps, is shown in Figure \maarteninline{add figure (placeholder if necessary -- to estimate how much space it takes up)}.

\subsection{Customization}\label{subsec:customization}
\maarten{Possibly, if space is limited, move to appendix or only include in camera ready}
In our main experiments, we considered one notion of toxicity as captured by the Jigsaw dataset and evaluated by Perspective API. 
However, different people have different notions of harmful language, and a good method for language avoidance should enable fine-grained control over the types of language being avoided. 
To approximate this desire for customizability, we explore steering away from four fine-grained types of toxic language: identity attacks, insults, sexual explicitness, and threats. 
These are the four subcategories of overlap between the Jigsaw dataset and the Perspective API toxicity classifier, providing us with the finetuning data and automatic evaluation we need. 

\maarten{These results are very intuitive and not surprising, so might potentially look like space filler to reviewers :/ }
Results in Table \ref{tab:toxicity_customization} show that the best way to avoid a certain type of toxicity is by using an anti-expert LM finetuned on that particular type of toxicity. 


